On the contribution of PRIDE-JUICE to Jovian system ephemerides

The JUICE mission will perform detailed measurements of the properties of the Galilean moons, with a nominal in-system science-mission duration of about 3.5 years. Using both the radio tracking data, and (Earth- and JUICE-based) optical astrometry, the dynamics of the Galilean moons will be measured to unprecedented accuracy. This will provide crucial input to the determination of the ephemerides and physical properties of the system, most notably the dissipation in Io and Jupiter. The data from Planetary Radio Interferometry and Doppler Experiment (PRIDE) will provide the lateral position of the spacecraft in the ICRF. In this article, we analyze the relative quantitative influence of the JUICE-PRIDE observables to the determination of the ephemerides of the Jovian system and the associated physical parameters. We perform a covariance analysis for a broad range of mission and system characteristics. We analyze the influence of VLBI data quality, observation planning, as well as the influence of JUICE orbit determination quality. This provides key input for the further development of the PRIDE observational planning and ground segment development. Our analysis indicates that the VLBI data are especially important for constraining the dynamics of Ganymede and Callisto perpendicular to their orbital planes. Also, the use of the VLBI data makes the uncertainty in the ephemerides less dependent on the error in the orbit determination of the JUICE spacecraft itself. Furthermore, we find that optical astrometry data of especially Io using the JANUS instrument will be crucial for stabilizing the solution of the normal equations. Knowledge of the dissipation in the Jupiter system cannot be improved using satellite dynamics obtained from JUICE data alone, the uncertainty in Io's dissipation obtained from our simulations is similar to the present level of uncertainty.

==> Figures2/tableOrbitPlanningRelativePositionUncertainty.tex <==
\begin{tabular}{r|l l|l l|l l|l l|l l}
\hline
\hline
& \multicolumn{10}{c}{Orbit Tracking Frequency}\\
\hline
& \multicolumn{2}{ c|}{Ganymede}& \multicolumn{2}{ c|}{Io}& \multicolumn{2}{ c|}{Europa}& \multicolumn{2}{ c|}{Callisto}& \multicolumn{2}{ c}{Jupiter}\\
Measurement case& IP & OP& IP & OP& IP & OP& IP & OP& IP & OP\\
\hline
Every week, $\sigma_{h}$=0.1 nrad &--&-16.8&--&--&--&--&--&--&-7.29&-15.2\\
$\sigma_{h}$=0.5 nrad &--&-45.8&--&--&--&--&--&--&--&-18.1\\
$\sigma_{h}$=1.0 nrad &--&-37.1&--&--&--&--&--&--&--&-14.5\\\hline
Every 3 months, $\sigma_{h}$=0.1 nrad &--&16.1&--&--&--&--&--&--&--&10.1\\
$\sigma_{h}$=0.5 nrad &--&12&--&--&--&--&--&--&--&7.97\\
$\sigma_{h}$=1.0 nrad &--&5.42&--&--&--&--&--&--&--&5.28\\\hline
Once, $\sigma_{h}$=0.1 nrad &--&103&--&--&--&--&--&12.5&5.59&42.8\\
$\sigma_{h}$=0.5 nrad &--&45.7&--&--&--&--&--&--&--&29.6\\
$\sigma_{h}$=1.0 nrad &--&15.8&--&--&--&--&--&--&--&19.1\\\hline
\end{tabular}

==> Figures2/tablePlanningRelativePositionUncertainty.tex <==
\begin{tabular}{r|l l|l l|l l|l l|l l}
\hline
\hline
& \multicolumn{10}{c}{Flyby Tracking Frequency}\\
\hline
& \multicolumn{2}{ c|}{Ganymede}& \multicolumn{2}{ c|}{Io}& \multicolumn{2}{ c|}{Europa}& \multicolumn{2}{ c|}{Callisto}& \multicolumn{2}{ c}{Jupiter}\\
Measurement case& IP & OP& IP & OP& IP & OP& IP & OP& IP & OP\\
\hline
Every flyby, $\sigma_{h}$=0.1 nrad &--&-13.6&--&--&--&-22.7&-9.6&-17.9&-11.9&-23.6\\
$\sigma_{h}$=0.5 nrad &--&-10.1&--&--&--&-9.02&--&-26.6&--&-21.3\\
$\sigma_{h}$=1.0 nrad &--&-5.52&--&--&--&--&--&-27.2&--&-20.8\\\hline
Every 3$^{rd}$ flyby, $\sigma_{h}$=0.1 nrad &--&--&--&--&--&--&--&--&--&--\\
$\sigma_{h}$=0.5 nrad &--&--&--&--&--&--&--&--&--&6.87\\
$\sigma_{h}$=1.0 nrad &--&--&--&--&--&--&--&--&--&8.98\\\hline
No Europa VLBI, $\sigma_{h}$=0.1 nrad &--&5.87&--&--&--&174&--&--&--&--\\
$\sigma_{h}$=0.5 nrad &--&--&--&--&--&15.8&--&--&--&--\\
$\sigma_{h}$=1.0 nrad &--&--&--&--&--&--&--&--&--&--\\\hline
No Ganymede flyby VLBI, $\sigma_{h}$=0.1 nrad &--&23.3&--&--&--&11.9&--&66.1&10.6&160\\
$\sigma_{h}$=0.5 nrad &--&9.71&--&--&--&--&--&29.1&--&146\\
$\sigma_{h}$=1.0 nrad &--&--&--&--&--&--&--&8.85&--&103\\\hline
No Callisto flyby VLBI, $\sigma_{h}$=0.1 nrad &--&23&--&--&--&--&104&2.07e+03&10.5&5.91\\
$\sigma_{h}$=0.5 nrad &--&--&--&--&--&--&91.8&541&6.01&--\\
$\sigma_{h}$=1.0 nrad &--&--&--&--&--&--&86.5&262&--&--\\\hline
No Ganymede VLBI, $\sigma_{h}$=0.1 nrad &--&396&--&--&--&54.3&--&273&22.7&403\\
$\sigma_{h}$=0.5 nrad &--&65.3&--&--&--&8.01&--&67.3&7.53&227\\
$\sigma_{h}$=1.0 nrad &--&20.8&--&--&--&--&--&16.2&8.67&161\\\hline
\end{tabular}
